B Lifetimes and Mixing

The Tevatron experiments, CDF and D0, have produced a wealth of new B-physics results since the start of Run II in 2001. We've observed new B-hadrons, seen new effects, and increased many-fold the precision with which we know the properties of b-quark systems. In these proceedings, we will discuss two of the most fruitful areas in the Tevatron B-physics program: lifetimes and mixing. We'll examine the experimental issues driving these analyses, present a summary of the latest results, and discuss prospects for the future.

==> Makefile <==
#----------------------------------------------------
# Generic make file for LaTeX: requires GNU make
#
# This makefile provides four targets: dvi, pdf and clean.
# The default is "pdf".
# To make a dvi file, type "make dvi"
# To make a pdf file, type "make pdf" or simply "make".
# To remove all files generated by make, type "make clean".
#
# original from:
# Rouben Rostmaian <rostamian@umbc.edu>
# September 2002
# http://www.math.umbc.edu/~rouben/prosper/large_sample/Makefile
#
# Modifications
# 03-Apr-07  add LATEX and DVIPDF
#-------------------------------------------------------

TEXFILE	= evans_hql08.tex
LATEX   = latex
DVIPDF  = dvipdfm
#DVIPDF  = dvipdf

.PHONY: dvi pdf

pdf:	$(TEXFILE:.tex=.pdf)
dvi:	$(TEXFILE:.tex=.dvi)

%.dvi: %.tex
	${LATEX} $<
	latex_count=5 ;\
	while grep 'Rerun to get cross-references right' $(TEXFILE:.tex=.log) && [ $$latex_count -gt 0 ] ;\
		do \
			${LATEX} $< ;\
			latex_count=`expr $$latex_count - 1` ;\
		done

%.pdf: %.dvi
	${DVIPDF} -o $(<:.dvi=.pdf) $<

clean:
	@rm -f \
	$(TEXFILE:.tex=.aux) \
	$(TEXFILE:.tex=.log) \
	$(TEXFILE:.tex=.out) \
	$(TEXFILE:.tex=.dvi) \
	$(TEXFILE:.tex=.pdf)

# DO NOT DELETE



